Random errors are not necessarily politically neutral

Errors are inevitable in the implementation of any complex process. Here we examine the effect of random errors on Single Transferable Vote (STV) elections, a common approach to deciding multi-seat elections. It is usually expected that random errors should have nearly equal effects on all candidates, and thus be fair. We find to the contrary that random errors can introduce systematic bias into election results. This is because, even if the errors are random, votes for different candidates occur in different patterns that are affected differently by random errors. In the STV context, the most important effect of random errors is to invalidate the ballot. This removes far more votes for those candidates whose supporters tend to list a lot of preferences, because their ballots are much more likely to be invalidated by random error. Different validity rules for different voting styles mean that errors are much more likely to penalise some types of votes than others. For close elections this systematic bias can change the result of the election.

==> ResponseToReviewers.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 47
TITLE: Random errors are not politically neutral
AUTHORS: Michelle Blom, Andrew Conway, Peter J. Stuckey, Vanessa Teague and Damjan Vukcevic

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The aim of the paper is to examine the effect of random errors on Single Transferable Vote (STV) elections. Research method is simulation of elections based on realistic random error rates. A main finding is that random errors can introduce systematic bias into election results. The paper discusses reasons for this effect along the experiments.
The paper is well organized and well written. The research method is presented clearly. The discussion of the reasons is comprehensible.
This investigation is important, because STV elections are frequently used. The paper dos not – but maybe should - provide suggestions how typical random errors could be avoided by electronic support during the ballot casting phase.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 47
TITLE: Random errors are not politically neutral
AUTHORS: Michelle Blom, Andrew Conway, Peter J. Stuckey, Vanessa Teague and Damjan Vukcevic

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The paper almost shows what the title claims: it shows that in some circumstances, for one particular voting rule, random errors that do not have a "direction" can still skew election results.

The paper makes its case well, but I suggest that, based on the evidence in the paper, a more accurate title would be "Random errors are not always politically neutral."

Author response: agreed - it's now "not necessarily..."

There are some issues that should be discussed (I am not suggesting additional analyses, just some discussion):

1. All the error models involve something like a "per rating" error process, which results in a larger chance of error for ballots that express more preferences. The authors should also discuss other models, for instance, "sloppy voters versus careful voters" which could be represented using something like a zero-inflated truncated Poisson model or zero-inflated negative binomial model.

Author response: good point.  We have added a comment about this ('voters with good handwriting vs voters with bad handwriting').
 
2. In ranked voting schemes, there is an obvious asymmetry: errors in interpreting the ranking of a candidate who is ranked 1 on the ballot can only hurt that candidate (directly or by causing the ballot to become invalid), while errors in interpreting the ranking of lower ranked candidates might help or hurt those candidates. This doesn't seem to be called out explicitly, but is implicit in one of the analyses.

Author response: this is mostly true, but STV is so complicated that it's hard to make a concrete statement about its implications.  For one thing, errors at a later preference can hurt the first-ranked candidate too (by invalidating the whole ballot), so we have left this observation out because it seems hard to make a general, true, summary.  (Don't even ask about monotonicity.  In STV, it isn't even true that cutting a candidate's first preferences can only hurt the candidate.)

3. While the paper is clearly of interest to Australians, some discussion of how this would carry over to plurality voting and other social choice functions seems to be in order. Certainly such discussion would seem to be required to justify the current title.

Author response: Thankyou, this is a very good point. We have added some ideas in the conclusion about how this might generalise.

The manuscript has a quite a few small grammatical issues that should be cleaned up (I've marked up the pdf extensively), but I'm not sure how to attach that to the review. One gaffe: there is no such thing as a "statistically significant random sample."

Author response: oops, now fixed.  Sorry we didn't see the pdf. We hope we've fixed most of the (other) bugs, but please send it if you find it.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 47
TITLE: Random errors are not politically neutral
AUTHORS: Michelle Blom, Andrew Conway, Peter J. Stuckey, Vanessa Teague and Damjan Vukcevic

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
Random errors are not politically neutral
-------------------------------------------

The paper simulates random errors in STV elections, using three error
models in which digits may be mis-written (or mis-read). It shows that
such random errors can have unexpected and apparantly biased
consequences. More precisely, it shows specific effects related to
Australian elections in which voters can vote either for a whole party
("above the line" (ATL)) or for specific candidates ("below the line"
(BTL)).


I think the research idea is interesting, and the paper is fairly
convincing. However, I have a few concerns:

- The paper concerns Australian elections only. This limits its
  impact. It would have been interesting to look more generally at STV
  elections (used all over the world).  The paper should make it clear
  in the title that its results apply to Australia specifically.

- The error models seem rather unrealistic, and contrived. Also, I
  couldn't figure them out exactly (either from their definition, or
  from their interpretation in the results section).

   * Error model 2. Why is the replacement digit randomly chosen? A
     "3" is more likely confused with a "8" than a "1".

   * What is the motivation for error model 3?
   
Author response: we agree that this was not very clear and have now tried to make it much clearer.  In fact, the third model that wasn't clear enough to this reviewer was exactly the 
pairwise error model that they (correctly) said was probably much more plausible.  


- The claim that random errors are not "politically" neutral seems
  invalid. While I can see that voters chosing BTL might be
  differently affected from those chosing ATL, this in itself is not a
  political distinction. I see no evidence, for example, that voters
  right-of-centre are affected differently by random errors to voters
  left-of-centre. So I recommend the title of the paper is changed,
  and the authors state their findings more carefully.

Author response: We don't think 'political' needs to be partisan - these errors clearly have political effects, so we are going to keep our title.


----------------------- REVIEW 4 ---------------------
SUBMISSION: 47
TITLE: Random errors are not politically neutral
AUTHORS: Michelle Blom, Andrew Conway, Peter J. Stuckey, Vanessa Teague and Damjan Vukcevic

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
The paper presents an interesting study of the influence of random errors during ballot processing on the final election result. The paper focuses on STV elections and the Australian setting in particular. Although it's not surprising that (uniformly) random errors do not have "uniformly" random consequences in an STV election, the study makes things very concrete and seems well-executed. 

So, a nice conference contribution. However, one major shortcoming is the lack of references overviewing related work. The current paper reads like an isolated study. Therefore, it's necessary to do a proper literature search. E.g., Google comes up with:

"Random and Systematic Error in Voting in Presidential Elections" by S. Richey, ‎2013

or another random hit: 

"Fraud or Human Error In Mexico’s Presidential Election?" by Javier Aparicio

and lots of other potentially relevant hits. Also other work that touches on the interplay of errors and elections can be included.


Author response: We've included the work from these suggestions that are closest to our work, but not all of them are close enough to warrant a ref.

Finally, it would be very nice if the study can be extended to cover other types of elections as well. Do you expect significant bias in other major forms of elections? Or mention it as an open question.

Author response: Good point - we have now added some ideas in the conclusion.

==> tables/formality-experiment.tex <==
\begin{tabular}{lrrrrrrrrr}
\toprule
  & \multicolumn{9}{c}{Number of BTL preferences required} \\
\cmidrule{2-10}
Per-digit error rate &
{\textbf{1}} & {\textbf{2}} & {\textbf{3}} & {\textbf{4}} & {\textbf{5}} & {\textbf{6}} & {\textbf{7}} & {\textbf{8}} & {\textbf{9}} \\ 
\midrule
  0.00\% &   0 &   0 &   0 &   0 &   0 &    0 &    0 &    0 &    0 \\ 
  0.05\% &   0 &   0 &   0 &   0 &   0 &    0 &    0 &    0 &    0 \\ 
  0.10\% &   0 &   0 &   0 &   0 &   0 &    0 &    0 &    0 &    0 \\ 
  0.15\% &   0 &   0 &   0 &   0 &   0 &    0 &    0 &    0 &    0 \\ 
  0.20\% &   0 &   0 &   0 &   0 &   0 &    0 &    0 &    0 &    0 \\ 
  0.25\% &   0 &   0 &   0 &   0 &   0 &    0 &    0 &    0 &    0 \\ 
  0.30\% &   0 &   0 &   0 &   0 &   0 &    0 &    5 &   11 &   25 \\ 
  0.35\% &   0 &   0 &   0 &   0 &   2 &   23 &   85 &  188 &  248 \\ 
  0.40\% &   0 &   0 &   0 &   0 &  19 &  144 &  335 &  403 &  475 \\ 
  0.45\% &   0 &   0 &   0 &   5 & 119 &  323 &  411 &  546 &  582 \\ 
  0.50\% &   0 &   0 &   0 &  32 & 254 &  431 &  638 &  732 &  812 \\ 
  0.55\% &   0 &   0 &   0 & 116 & 274 &  592 &  827 &  876 &  928 \\ 
  0.60\% &   0 &   0 &  10 & 155 & 443 &  780 &  911 &  962 &  979 \\ 
  0.65\% &   0 &   0 &  27 & 218 & 602 &  878 &  972 &  982 &  992 \\ 
  0.70\% &   0 &   0 &  61 & 286 & 728 &  939 &  990 &  998 &  999 \\ 
  0.75\% &   0 &   0 &  65 & 451 & 857 &  974 &  995 & 1000 & 1000 \\ 
  0.80\% &   0 &   2 & 107 & 607 & 923 &  990 &  999 & 1000 & 1000 \\ 
  0.85\% &   0 &   2 & 172 & 689 & 953 &  994 & 1000 & 1000 & 1000 \\ 
  0.90\% &   0 &  11 & 226 & 760 & 976 &  997 & 1000 & 1000 & 1000 \\ 
  0.95\% &   0 &  14 & 307 & 852 & 989 &  999 & 1000 & 1000 & 1000 \\ 
  1.00\% &   0 &  19 & 392 & 897 & 997 & 1000 & 1000 & 1000 & 1000 \\ 
\bottomrule
\end{tabular}

